Adversarial Examples Exist in Two-Layer ReLU Networks for Low Dimensional Linear Subspaces

Despite a great deal of research, it is still not well-understood why trained neural networks are highly vulnerable to adversarial examples. In this work we focus on two-layer neural networks trained using data which lie on a low dimensional linear subspace. We show that standard gradient methods lead to non-robust neural networks, namely, networks which have large gradients in directions orthogonal to the data subspace, and are susceptible to small adversarial $L_2$-perturbations in these directions. Moreover, we show that decreasing the initialization scale of the training algorithm, or adding $L_2$ regularization, can make the trained network more robust to adversarial perturbations orthogonal to the data.

==> appen_proofs_from_setting.tex <==
\section{Proofs from \secref{frameworksection}}\label{apen:proofs from settings}


\begin{proof}[Proof of \thmref{thm:small margin}]
For a data point $\bx_i\in X$ we denote by $\hat{y}_i:= N(\bx_i)$. The derivative of the logistic loss over a single point $\bx_i$ w.r.t a single weight vector $\bw_j$ is:

\[
\frac{\partial \ell(y,\hat{y}_i)}{\partial \bw_j}=  \frac{\partial \ell(y,\hat{y}_i)}{\partial\hat{y}}\cdot \frac{\partial \hat{y}_i}{\partial \bw_j} = \frac{-y  e^{-y\hat{y}_i}}{1+e^{-y\hat{y}_i}}\cdot \frac{\partial N(\bx_i)}{\partial \bw_j} 
\]
The norm of $\frac{\partial N(\bx_i)}{\partial \bw_j} $ can be bounded in the following way:

\[
\norm{\frac{\partial N(\bx_i)}{\partial \bw_j} } = \norm{\sum\limits_{k=1}^{m} u_i\cdot \frac{\partial \sigma(\inner{\bw_k,\bx_i})}{\partial \bw_j}} \leq  \norm{u_j \sigma'(\bw_j^\top \bx_i) \bx_i} \leq |u_j|\cdot \norm{\bx_i} = \frac{\norm{\bx_i}}{\sqrt{m}} 
\]
% We look at BCE loss for a data point $x$ labeled as $y$ and denote $\hat{y} = N(x)$. Recall that our loss and its derivative are:

% % $$L_{BCE} = y log(\hat{y}) + (1-y)log(1-\hat{y})$$

% % $$\Delta = \frac{\delta L_{BCE}}{\delta\hat{y}} = y \frac{1}{\hat{y}} + (1-y) (-\frac{1}{1-\hat{y}})$$


% \[L_{BCE} = log(1+e^{-y\hat{y}})\]



% % $$\Delta = \frac{\delta L_{BCE}}{\delta\hat{y}} = \frac{-y  e^{-y\hat{y}}}{1+e^{-y\hat{y}}} $$

% \[\frac{\partial L_{BCE}}{\partial w}=  \frac{\partial L_{BCE}}{\partial\hat{y}}\cdot \frac{\partial \hat{y}}{\partial w} = \frac{-y  e^{-y\hat{y}}}{1+e^{-y\hat{y}}}\cdot \frac{\partial N(x)}{\partial w} \]


% \[
% \left|\frac{\partial N(x)}{w_i}\right| = |u_i\cdot \sigma'(\inner{w_i,x})x| \leq \frac{\norm{x}}{\sqrt{m}}
% \]

For the dataset $X$ of size $K$, the loss of a gradient step over all the data, w.r.t all the weights of the first layer, denoted by $\bw_1^m$ (which can be viewed as a concatenation of $\bw_1,\dots,\bw_m$) can be bounded by: 

\begin{align*}
    \norm{\frac{1}{K}\sum_{i=1}^K \frac{\partial \ell(y,\hat{y}_i)}{\partial \bw_1^m}} &\leq \norm{\frac{1}{K}\sum_{i=1}^K \frac{N(\bx_i)}{\partial \bw_1^m}} \cdot \left|\frac{1}{K}\sum_{i=1}^K\frac{\partial \ell(y,\hat{y}_i)}{\partial \hat{y_i}} \right| \\
    &\leq \frac{1}{K}\sum_{i=1}^K\sum_{j=1}^m\norm{\frac{\partial N(\bx_i)}{\partial \bw_j} }\cdot \left|\frac{1}{K}\sum_{i=1}^K\frac{\partial \ell(y,\hat{y}_i)}{\partial \hat{y_i}} \right|\\
    & \leq  \frac{\sqrt{m}\sum_{i=1}^K\norm{x_i}}{K} \cdot \frac{1}{K}\sum\limits_{i=0}^K \left|\frac{-y_i   e^{-y_i\hat{y_i}}}{1+e^{-y_i\hat{y_i}}}\right|  
\end{align*}
% \[
% \leq \sqrt{m} \norm{x_i} \cdot \frac{1}{K}\sum\limits_{i=0}^k \left|\frac{-y_i   e^{-y_i\hat{y_i}}}{1+e^{-y_i\hat{y_i}}}\right|  
% % = \sum\limits_{i=0}^B -y \cdot e^{-y_i\hat{y_i}}\frac{1}{1+e^{-y_i\hat{y_i}}}
% \]
If the classification output of the network after the gradient step is correct for all $\bx_i \in X$, we get that for all $i \in [K]$:
\[
\left|\frac{-y_i   e^{-y_i\hat{y_i}}}{1+e^{-y_i\hat{y_i}}} \right|\leq \frac{ e^{-\gamma}}{1+e^{-\gamma}} \leq \frac{e^{-\gamma}}{2}
\]
Combining the last two equations, we can bound the gradient of the loss w.r.t all the weights by 
\[
    \frac{\sqrt{m}\sum_{i=1}^K\norm{x_i}}{2K}\cdot e^{-\gamma}
\]
Note that if there is at least one point which the network does not classify correctly after the gradient step, then the margin must be $0$ by our definition, hence the margin did not increase.
% \[
% \norm{\frac{\partial L_{BCE}}{\partial w}} \leq \sqrt{m} \norm{x_i} \frac{e^{-\gamma}}{2}
% \]
Denote by $\eta$ the learning rate, and denote $C:=\eta\cdot  \frac{\sqrt{m}\sum_{i=1}^K\norm{x_i}}{2K}$. By calculations above we can bound the change of the margin after $T$ iterations in the following way:
\begin{align*}
    \gamma_{T} &\leq \gamma_{T-1} + C\cdot e^{-\gamma_{T-1}}\\
    &\leq \dots \leq \gamma_0 + C\cdot \sum_{t=1}^{T-1}e^{-\gamma_t}
\end{align*}
We will show that $\gamma_{T} \leq \gamma_0 + O(\poly\log(d))$ using induction over $t$. For $t=0$ it is clear. Assume it is true for $t-1$, then:
\[
\gamma_t \leq \gamma_0 + C\cdot \sum_{i=1}^{t-1} e^{-\gamma_i}
\]
Note that by our assumption


TODO: why does this imply low margin increase.
If we use a gradient step size bounded by a constant $C$ for training and denote the margin after training step $t$ by $\gamma_t$ we get that in each step, we can increase the margin by at most $C \cdot \sqrt{m} \norm{x_i} \frac{e^{-\gamma}}{2}$. Meaning:

\[
\gamma_{t+1} \leq \gamma_t + C \cdot \sqrt{m} \norm{x_i} \frac{e^{-\gamma_t}}{2}
\]

\paragraph{Using O notations:}
Using $O$ notation we get that $\gamma_{t+1} = \gamma_t + O(d e^{-\gamma_t})$. If in all training iterations $t$, $\gamma_t = o(log^2d)$, than $\gamma_T = o(log^2d) = O(polylog(d))$.
Else, there exists $t$ for which $\gamma_t = \Omega(log^2d)$, then it won't increase further:
even $ T = poly(d)$ steps, will cause almost no change in the margin:

\[ \gamma_{t+T} = \gamma_t + O(T \cdot \frac{d}{d^{logd}}) = \gamma_t + O(\frac{d\cdot poly(d)}{d^{logd}}) \]
One can see that \[ \frac{poly(d)}{d^{logd}} \xrightarrow{d \to \infty} 0\]
and the claim follows.

\end{proof}

==> z02smallmargin.tex <==
\section{Small margin}

For a network $N$ and a dataset $X$ defined in \secref{frameworksection}, we define the margin of a network $N$ as $\gamma = \min_{x \in X} N(x)$.
\begin{theorem}
Let the network $N(x) = \sum\limits_{i=1}^{m} u_i \sigma(w_i^Tx) $, initialized and trained as described in \secref{frameworksection}, with the standard BCE loss on data $X$ lies on a $d-\ell$ dimensional linear manifold $P \subset \reals^d$ and binary labels $\{-1, 1\}$. Denote the margin in the initialization by $\gamma_0$, and the margin after training step $t$ by $\gamma_t$. Note, where at least one point is misclassified by the network, $\min_{x \in X} N(x) < 0$.\\

Assume that for all $x \in X$, $\norm{x} = O(\sqrt{d})$, $m = O(d)$ and that after training, all the training data points are labeled correctly by $N$. Then, After $T$ training iterations, the margin will not increase by more than O(log(T)).
\[
\gamma_T = \gamma_0 + O(log(T))
\]

In particular, if we train for $T=\text{poly}(d)$ iterations, then $\gamma_T = \gamma_0 + O(\text{polylog}(d))$
    % After $T= poly(d)$ training steps, assuming all the training set is classified correctly by $N$, the margin is $\gamma = polylog(d)$ 
\end{theorem}

%change that you cannot add more that polylog, margin is negative is there is any data point we missclassifier, so it is max(0, \gamma_0) is probably 0.

%sum going to upper bound - |sum| < = sum|| and that there is upper bound
%batch B be raplced with training data size, and then avg by 1/data size

% add the gradient of the network, bounded bt |x| / sqrt m, which is O(1) and can be input to C
% C need to be upper bound for the step size
% to the thm, data is size sqrtd, and m is O(d), and the setting of the network, training and init like is prelimieries.
%save the O notation to the end

\begin{proof}
We look at BCE loss for a data point $x$ labeled as $y$ and denote $\hat{y} = N(x)$. Recall that our loss and its derivative are:

% $$L_{BCE} = y log(\hat{y}) + (1-y)log(1-\hat{y})$$

% $$\Delta = \frac{\delta L_{BCE}}{\delta\hat{y}} = y \frac{1}{\hat{y}} + (1-y) (-\frac{1}{1-\hat{y}})$$


\[L_{BCE} = log(1+e^{-y\hat{y}})\]



% $$\Delta = \frac{\delta L_{BCE}}{\delta\hat{y}} = \frac{-y  e^{-y\hat{y}}}{1+e^{-y\hat{y}}} $$

\[\frac{\partial L_{BCE}}{\partial w}=  \frac{\partial L_{BCE}}{\partial\hat{y}}\cdot \frac{\partial \hat{y}}{\partial w} = \frac{-y  e^{-y\hat{y}}}{1+e^{-y\hat{y}}}\cdot \frac{\partial N(x)}{\partial w} \]

Note, the norm of $\frac{\partial N_w(x)}{\partial w}$ can be bounded:

\[
\norm{\frac{\partial N(x)}{ \partial w}} = \norm{\sum\limits_{i=1}^{m} u_i\cdot \sigma'(\inner{w_i,x})x} \leq  \norm{\sum\limits_{i=1}^{m} u_i x} \leq \sum\limits_{i=1}^{m} |u_i| \norm{x} = m \frac{1}{\sqrt{m}} \norm{x} = \sqrt{m} \norm{x}
\]

% \[
% \left|\frac{\partial N(x)}{w_i}\right| = |u_i\cdot \sigma'(\inner{w_i,x})x| \leq \frac{\norm{x}}{\sqrt{m}}
% \]

For the dataset $X$ of size $K$ ($x_1,..,x_K$ with labels $y_1,...,y_K$) we define $\hat{y_i} = N(x_i)$.  The loss is $\frac{1}{K} \sum\limits_{i=0}^K log(1+e^{-y_i\hat{y_i}})$
and the gradient will be: 

\[ \norm{\frac{\partial L_{BCE}}{\partial w}} = \norm{\frac{\partial N(x_i)}{ \partial w}} \cdot \left|\frac{1}{K} \sum\limits_{i=0}^K \frac{-y_i   e^{-y_i\hat{y_i}}}{1+e^{-y_i\hat{y_i}}}\right| \leq \]


\[
\leq \sqrt{m} \norm{x_i} \cdot \frac{1}{K}\sum\limits_{i=0}^k \left|\frac{-y_i   e^{-y_i\hat{y_i}}}{1+e^{-y_i\hat{y_i}}}\right|  
% = \sum\limits_{i=0}^B -y \cdot e^{-y_i\hat{y_i}}\frac{1}{1+e^{-y_i\hat{y_i}}}
\]

if the classification is correct for all $x_i \in X$, we get that for all $i \in [K]$:

\[
\frac{-y_i   e^{-y_i\hat{y_i}}}{1+e^{-y_i\hat{y_i}}} \leq \frac{-y \cdot e^{-\gamma}}{1+e^{-\gamma}} \leq \frac{e^{-\gamma}}{2}
\]

Combining the last two equations, we get:
\[
\norm{\frac{\partial L_{BCE}}{\partial w}} \leq \sqrt{m} \norm{x_i} \frac{e^{-\gamma}}{2}
\]
TODO: why does this imply low margin increase.
If we use a gradient step size bounded by a constant $C$ for training and denote the margin after training step $t$ by $\gamma_t$ we get that in each step, we can increase the margin by at most $C \cdot \sqrt{m} \norm{x_i} \frac{e^{-\gamma}}{2}$. Meaning:

\[
\gamma_{t+1} \leq \gamma_t + C \cdot \sqrt{m} \norm{x_i} \frac{e^{-\gamma_t}}{2}
\]

\paragraph{Using O notations:}
Using $O$ notation we get that $\gamma_{t+1} = \gamma_t + O(d e^{-\gamma_t})$. If in all training iterations $t$, $\gamma_t = o(log^2d)$, than $\gamma_T = o(log^2d) = O(polylog(d))$.
Else, there exists $t$ for which $\gamma_t = \Omega(log^2d)$, then it won't increase further:
even $ T = poly(d)$ steps, will cause almost no change in the margin:

\[ \gamma_{t+T} = \gamma_t + O(T \cdot \frac{d}{d^{logd}}) = \gamma_t + O(\frac{d\cdot poly(d)}{d^{logd}}) \]
One can see that \[ \frac{poly(d)}{d^{logd}} \xrightarrow{d \to \infty} 0\]
and the claim follows.

\end{proof}







==> z05smallinitialization.tex <==
\section{Small initialization and robustness}

\subsection{upper bound for the norm of the projected gradient}







\subsection{Small initialization induce small gradient norm}
\begin{corollary}
Let the network $N(x) = \sum\limits_{i=1}^{m} u_i \sigma(w_i^Tx) $ for $w_i$ initialized from $\mathcal{N}(0,\beta\frac{1}{\sqrt{d}})$, trained on dataset $X$ which lies on linear subspace $P \subset \reals^d$ of dimension $d-\ell$ for $\ell \geq 1$, and let $x_0 \in P$. Let $S= \{i\in[m]: w_i^\top x_0 \geq 0\}$, and let $k := |S|$.
    %   We say that a neuron $i\in[m]$ is active w.r.t $x_0$ if $w_i^\top x_0 \geq 0$. Let $S\subseteq [m]$ be the set of active neurons of $N$ w.r.t $x_0$, and let $k = |S|$. 
    %   Let $\hat{x}_0 = \Pi_{P^\perp}\left(x_0\right)$ be the projection of $x_0$ on $P^\perp$ (the subspace orthogonal to $P$), and define  $\Pi_{P^\perp} \left(\frac{\partial N(x_0)}{\partial x_0}\right)$ be the projection of the gradient of $N$ w.r.t $x_0$ on $P^\perp$.
    Then, w.p $\geq 1 - e^{-\frac{n}{16}}$ we get:
    \[\norm{\Pi_{P^\perp}\left(\frac{\partial N(x_0)}{\partial x_0}\right)} \leq \sqrt{2} \beta \sqrt{\frac{k l}{ m d}}~. \]

During the proof of \thmref{small initialization gradient}, one can see that the parameter $d$ is used only as the initialization weight (since $l$ is the effective dimension of the projected vectors). If we initialized the coordinates of the weights vector as $w_i \sim \mathcal{N}(0,\beta\frac{1}{\sqrt{d}})$ for some $\beta \in (0,1)$ we get that the upper bound on the norm of the projected gradient is tighter:

\[\norm{\Pi_{P^\perp}\left(\frac{\partial N(x_0)}{\partial x_0}\right)} \leq \sqrt{2} \beta \sqrt{  \frac{k l}{ m d}} \leq \sqrt{2} \sqrt{\frac{k l}{ m d}}  ~. \]
\end{corollary}
\subsection{Small initialization effects suggested adversarial perturbation}
?

==> z06explicitregularization.tex <==
\section{Explicit $L_2$ regularization and robustness}
In this section, we show that a $L_2$ regularization on the weights will increase the lower bound on the projected gradient. When introducing an $L_2$ regularization, we revisit the training process of the projected weights vectors $\Pi_{M^\perp}\left(w_i\right) = \hat{w}_i$ for $i \in [m]$. For a data point $x$ labeled as $y$, we denote $\hat{y} = N(x)$ and define the loss function w.r.t the weight vector $w_i$: $\ell_R(y,\hat{y}, w_i) = \log(1+e^{-y\hat{y}}) + \lambda \norm{w_i}$. 

In \thmref{thm:weights dont change}, we showed the gradient of the network on a point $x$ on the manifold $M$ w.r.t the weights, relevant to the training process: 

\[\frac{\partial N(x)}{\partial w_i} = u_i  \sigma'(w_i^\topx) (w_i^\topx)' = u_i  \sigma'(w_i^\topx) x. \]
where
\[\frac{\partial L_{BCE}}{\partial w_i}=  \frac{\partial L_{BCE}}{\partial\hat{y}}\cdot \frac{\partial \hat{y}}{\partial w_i} = \frac{-y  e^{-y\hat{y}}}{1+e^{-y\hat{y}}}\cdot \frac{\partial N(x)}{\partial w_i}.\]

And we showed that the projection of the weight vector $\Pi_{M^\perp}\left(w_i\right) = \hat{w}_i$ does not change during training.
When considering the new loss including regularization we get that the projected weights are also affected during training, since:

\[\frac{\partial \ell_R}{\partial w_i} = \frac{\partial L_{BCE}}{\partial\hat{y}}\cdot \frac{\partial \hat{y}}{\partial w_i} + \frac{\partial \lambda \norm{w_i}}{\partial w_i}.\]

We denote by $w^t_i$ the weight vector $w_i$ after $t$ training steps, and by $\Pi_{M^\perp}\left(w^t_i\right) = \hat{w}^t_i$ its projection on the subspace orthogonal to the data manifold.
We look at the projected gradient of $w^t_i$ w.r.t to the new loss:

\begin{align*}
    \Pi_{M^\perp}\left(\frac{\partial \ell_R}{\partial w^t_i}\right) =& \Pi_{M^\perp}\left(\frac{\partial L_{BCE}}{\partial\hat{y}}\cdot \frac{\partial \hat{y}}{\partial w^t_i}\right) + \Pi_{M^\perp}\left(\frac{\partial \lambda \norm{w^t_i}}{\partial w^t_i}\right)\\
    =& \Pi_{M^\perp}\left(\frac{\partial \lambda \norm{w^t_i}}{\partial w^t_i}\right) = \lambda \hat{w^t}_i 
\end{align*}

For a training step size of size $\eta$, using the gradient descent training method, we get that:

\[ \hat{w}^{t+1}_i = \hat{w}^{t}_i + \eta \lambda \hat{w^t}_i.  \]

Thus, after a total of $T$ iteration of training with training step upper bounded by $\eta$ we get that for a constant $B \leq (1- \eta \lambda)^\top$:

\[ \hat{w}^{T}_i = B \hat{w}^{0}_i  \].

If we look at the projected gradient of the network w.r.t. to the input $x$, we can see that this case is similar to the case of small initialization of the weights \thmref{small initialization gradient} for $B=\beta$. Similarly, one can prove that:  
\begin{theorem}
\label{explicit regularization gradient}
       Let the network $N(x) = \sum\limits_{i=1}^{m} u_i \sigma(w_i^\topx) $, trained with logistic loss with $\lambda$ $L_2$ regularization and step size bounded by $\eta$, on dataset $X$ which lies on linear subspace $P \subset \reals^d$ of dimension $d-\ell$ for $\ell \geq 1$ , and let $x_0 \in P$. Let $S= \{i\in[m]: w_i^\top x_0 \geq 0\}$, and let $k := |S|$.
    %   We say that a neuron $i\in[m]$ is active w.r.t $x_0$ if $w_i^\top x_0 \geq 0$. Let $S\subseteq [m]$ be the set of active neurons of $N$ w.r.t $x_0$, and let $k = |S|$. 
    %   Let $\hat{x}_0 = \Pi_{P^\perp}\left(x_0\right)$ be the projection of $x_0$ on $P^\perp$ (the subspace orthogonal to $P$), and define  $\Pi_{P^\perp} \left(\frac{\partial N(x_0)}{\partial x_0}\right)$ be the projection of the gradient of $N$ w.r.t $x_0$ on $P^\perp$.
    Then, for $B \leq (1- \eta \lambda)^\top$, w.p $\geq 1 - e^{-\frac{n}{16}}$ we get:
    \[\norm{\Pi_{P^\perp}\left(\frac{\partial N(x_0)}{\partial x_0}\right)} \leq \sqrt{2} B \sqrt{\frac{k l}{ m d}}~. \]

 %we need oproject the geadient
\end{theorem}







